X*: Anytime Multi-Agent Path Finding for Sparse Domains using Window-Based Iterative Repairs

Real-world multi-agent systems such as warehouse robots operate under significant time constraints -- in such settings, rather than spending significant amounts of time solving for optimal paths, it is instead preferable to find valid collision-free paths quickly, even if suboptimal, and given additional time, to iteratively refine such paths to improve their cost. In such domains, we observe that agent-agent collisions are sparse -- they involve small local subsets of agents, and are geographically contained within a small region of the overall space. Leveraging this insight, we can first plan paths for each agent individually, and in the cases of collisions between agents, perform small local repairs limited to local subspace windows. As time permits, these windows can be successively grown and the repairs within them refined, thereby improving the path quality, and eventually converging to the global joint optimal solution. Using these insights, we present two algorithmic contributions: 1) the Windowed Anytime Multiagent Planning Framework (WAMPF) for a class of anytime planners that quickly generate valid paths with suboptimality estimates and generate optimal paths given sufficient time, and 2) X*, an efficient WAMPF-based planner. X* is able to efficiently find successive valid solutions by employing re-use techniques during the repair growth step of WAMPF. Experimentally, we demonstrate that in sparse domains: 1) X* outperforms state-of-the-art anytime or optimal MAPF solvers in time to valid path, 2) X* is competitive with state-of-the-art anytime or optimal MAPF solvers in time to optimal path, 3) X* quickly converges to very tight suboptimality bounds, and 4) X* is competitive with state-of-the-art suboptimal MAPF solvers in time to valid path for small numbers of agents while providing much higher quality paths.

==> astar.tex <==
\section{A*}\sectionlabel{astar}

The A* algorithm~\cite{astar} is a combinatorial search algorithm that produces and
utilizes data structures which uphold specific properties. We present a variant of A* along with novel
formalization of these properties. We prove that these properties are upheld by our variant of A*.
%, and show these properties are useful by using them to prove fundamental, previously known results about A*.

\subsection{The A* Algorithm}\subsectionlabel{AStarAlgo}

The pseudocode for our variant of A* is provided in \algoref{AStar} using the definitions from
\sectionref{Definitions}. Note that, for convenience,
we define $\topopenset{\start}{\goal}$ to be the state with the smallest
\fvalue{}, i.e. $\topopenset{\start}{\goal} := \state \in \openset: \argmin
\f{\state}{\start}{\goal}$. In addition, \Call{UnwindPath}{} (\lineref{AStarUnwind}) operates by taking a current state, initialized to $\goal$, and repeatedly taking the neighbor which has the lowest \gvalue{} until the current state is $\start$, thereby producing a minimal cost path from $\goal$ to $\start$, which is then reversed. Our variant of A* differs from other presentations of A* as it updates the \gvalue{} of neighbor states when they are added to $\openset{}$ (\lineref{AStarSetGValue}) rather than when the state is expanded (\lineref{AStarAccessTop}) in order to ensure that all states in $\openset$ have a finite \gvalue{}. Furthermore, note that $\openset$ is a set and thus  \lineref{AStarAddStateToOpenSet} handles de-duplication of states in $\openset$.


\begin{algorithm}
  \caption{A*}\algolabel{AStar}
  \begin{algorithmic}[1]
    \Function{A*}{$\start, \goal$}
    \State $\openset \gets \{\start\}$\linelabel{AStarInitOpenSet}
    \State $\g{\start}{\start} = 0$
    \State $\closedset \gets \emptyset$\linelabel{AStarInitClosedSet}
    \While{$\openset \neq \emptyset$}\linelabel{AStarStart}
    \State $\state \gets \topopenset{\start}{\goal}$\linelabel{AStarAccessTop} \linelabel{AStarLoopStart}
    \If{$\state = \goal$}
    \Return \Call{UnwindPath}{$\closedset, \goal, \start$}\linelabel{AStarUnwind}
    \EndIf
    \State $\openset \gets \openset \setminus \{\state\}$\linelabel{AStarRemoveState}
    \If{$\state \in \closedset$}
    \Continue
    \EndIf\linelabel{AStarInClosed}
    \State $\closedset \gets \closedset \cup \{\state\}$\linelabel{AStarCloseState}
    \ForAll{$\state' \in \neighbors{\state}\setminus \closedset$}\linelabel{AStarNeighborLoop}
    \State $\openset \gets \openset \cup \{\state'\}$\linelabel{AStarAddStateToOpenSet}
    \State $\g{\state'}{\start} \gets \min \left( \g{\state'}{\start} ,
      \g{\state}{\start}+ \cost{\state}{\state'} \right)$\linelabel{AStarSetGValue}
    \EndFor
    \EndWhile \linelabel{AStarLoopEnd}
    \State \Return \nopath{}\linelabel{AStarNOPATH}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\subsection{\astarsearchtree{s} and Valid Search Tree Properties}\subsectionlabel{SearchTreeProperty}

A* constructs \emph{\astarsearchtree{s}}. These search trees are comprised
of two sets of states, an open set $\openset$ and a closed set $\closedset$,
which store the information used in a search to find shortest paths.
For an \astarsearchtree{} to be considered \emph{valid} given a start $\start$ and a
goal $\goal$, the following \emph{Valid Search Tree Properties} (\vstps{})
must hold at the beginning of each A* expansion loop (\lineref{AStarStart}) or when a path is produced (\lineref{AStarUnwind} or \lineref{AStarNOPATH}):

% \propertylabel{AStarStartInTree}\\
% \propertylabel{AStarHasMinimalParent} \\
% \propertylabel{AStarNeighborsNotDropped}\\
% \propertylabel{AStarPathExists}\\
% \propertylabel{AStarFValueProperlyOrdered}

\begin{align}
  &\start \in \openset \cup \closedset\propertylabel{AStarStartInTree}\\
  &\forall \state \in \openset \cup \closedset: \state \neq \start \implies \exists \state': \begin{cases} 
  \state' \in \closedset\\
  \state' = \argmin_{\state'' \in \neighbors{\state}} \g{\state''}{\start} + \cost{\state''}{\state}\\
  \g{\state'}{\start} + \cost{\state'}{\state} = \g{\state}{\start}
\end{cases}\propertylabel{AStarHasMinimalParent} \\
  &\forall \state \in \closedset: \neighbors{\state} \subseteq \openset \cup \closedset \propertylabel{AStarNeighborsNotDropped}\\
  &\forall \state \in \openset \cup \closedset  : \exists \pth: \pth_1 = \start \land \pth_{\len{\pth}} = \state \land \forall \state' \in \pth: \state' \neq \state \implies \state' \in \closedset  \propertylabel{AStarPathExists}\\
  &\forall \state \in \closedset, \forall \state' \in \openset: \f{\state}{\start}{\goal} \leq \f{\state'}{\start}{\goal}\propertylabel{AStarFValueProperlyOrdered}
\end{align}

Intuitively, \propertyref{AStarStartInTree} says that $\start$ must always be in the search tree. \propertyref{AStarHasMinimalParent} says that all states $\state$ in $\openset$ or $\closedset$ which are not $\start$ have a parent $\state'$ where $\state' \in \closedset$, $\state'$ is on the minimal cost path to $\state$, and the lowest cost to reach $\state$ is the cost of reaching $\state'$ and then moving to $\state$. \propertyref{AStarNeighborsNotDropped} says that all states in $\closedset$ must have placed all their neighbors in the $\openset$ or $\closedset$. \propertyref{AStarPathExists} says that all states in $\openset$ or $\closedset$ must have a path to $\start$, and all states along the way must be in $\closedset$. \propertyref{AStarFValueProperlyOrdered} says that \fvalue{} ordering must be maintained between all states in $\openset$ and $\closedset$.
We prove that A* upholds these properties in \theoremref{AStarValidSearchTree} in \appendixref{astarsearchtreeproofs}. 

% As a consequence of these properties, the following theorems hold
% for all \astarsearchtree{s} where \vstps{} hold at the beginning of each A* expansion loop (\lineref{AStarStart}) or when a path is produced (\lineref{AStarUnwind} or \lineref{AStarNOPATH}):

% \begin{theorem}\theoremlabel{AStarValidSearchTree}
% Given a consistent heuristic, A* produces valid \astarsearchtree{s}.
% \end{theorem}

% \begin{theorem}\theoremlabel{PathNonDecrease}

% Given a consistent heuristic and an optimal path $\pth$ from $\start$ to $\goal$, the \fvalue{s} along the
% path are non-decreasing, i.e.\ $\forall i:
% \f{\pth_i}{\start}{\goal} \leq \f{\pth_{i+1}}{\start}{\goal}.$
  
% \end{theorem}

% \begin{theorem}\theoremlabel{FValueInClosedSet}
%   $\forall \state \in \closedset, \forall \state', \exists \pth: ( \pth_1 =
%     \start \land \pth_{\len{\pth}} = \state' ) \land (
%     \pthcost{\pth} + \h{\state'}{\goal}  <
%   \f{\state}{\start}{\goal}) \implies \state' \in \closedset$
% \end{theorem}

% \begin{theorem}\theoremlabel{VSPTClosedStateOptimal}
%   Given a consistent heuristic and a valid \astarsearchtree{} with a start $\start$, we know the optimal
%   path from $\start$ to all states in $\closedset$.
% \end{theorem}

% \noindent Proofs are provided in \appendixref{astarsearchtreeproofs}.

% \subsection{Fundamental A* Results}\subsectionlabel{AStarProperties}

% In order to utilize the theorems we proved in \subsectionref{SearchTreeProperty}
% on the output of A*, we must prove that A* produces \astarsearchtree{s} which
% uphold the \vstps{}. Once we prove that A* produces valid \astarsearchtree{s},
% we can then use the \vstps{} to prove properties about the output of A*.

% \begin{theorem}

% If we assume  the heuristic is
% consistent, then the path A* produces an optimal path from $\start$ to $\goal$.
% \end{theorem}

% \begin{theorem}
% If we assume  the heuristic is consistent, A* is \emph{complete},
% i.e.\ will find a solution if it exists.
% \end{theorem}


% \begin{theorem}
%   If we assume  the heuristic is consistent, A* is
%   \emph{optimally efficient}, i.e.\ no other search algorithm can expand fewer
%   states, barring tie-breaking, and still be complete.
% \end{theorem}

% \noindent Proofs are provided in \appendixref{astarproofs}.
